A Survey on Perfectly-Secure Verifiable Secret-Sharing

Verifiable Secret-Sharing (VSS) is a fundamental primitive in secure distributed computing. It is used as a building block in several distributed computing tasks, such as Byzantine agreement and secure multi-party computation. In this article, we consider VSS schemes with perfect security, tolerating computationally unbounded adversaries. We comprehensively survey the existing perfectly-secure VSS schemes in three different communication settings, namely synchronous, asynchronous and hybrid setting and provide full details of the existing schemes in these settings. The aim of this survey is to provide a clear knowledge and foundation to researchers who are interested in knowing and extending the state-of-the-art perfectly-secure VSS schemes.

==> Figures/WSSToVSS.tex <==
\begin{figure}[!h]
  \centering
  \hspace*{-1cm}%
  \begin{tikzpicture}[scale=0.85]
    %% Polynomial (a)
    % Main rectangle
    \draw (0, 0) rectangle (7, 5);
    % Columns
    \draw (0, 2) -- (7, 2);
    \draw (0, 3) -- (7, 3);
    \draw (2.75, 0) -- (2.75, 5);
    \draw (4.25, 0) -- (4.25, 5);
    % Coloured Rectangles
    \draw [rounded corners, fill=ForestGreen!30] (8, 0) rectangle (9, 5);
    \draw [rounded corners, fill=DarkRed!30] (0, -2) rectangle (7, -1);
    % Annotations
    \draw (3.5, -4) node {\footnotesize (a)};
    % ---
    \draw (-1, 2.5) node {\footnotesize $f_i(x)$};
    \draw (-0.3, 2.5) node {\footnotesize $\Rightarrow$};
    \draw (3.5, 6) node {\footnotesize $g_i(y)$};
    \draw (3.5, 5.5) node {\footnotesize $\Downarrow$};
    % ---
    \draw (1, 4.5) node {\scriptsize $F(\alpha_1, \alpha_1)$};
    \draw (2.25, 4.5) node {\scriptsize $\ldots$};
    \draw (3.5, 4.5) node [text=ForestGreen] {\tiny $\boldsymbol{F(\alpha_i, \alpha_1)}$};
    \draw (4.75, 4.5) node {\scriptsize $\ldots$};
    \draw (6, 4.5) node {\scriptsize $F(\alpha_n, \alpha_1)$};
    % ---
    \draw (1, 3.5) node {\scriptsize $\rvdots$};
    \draw (2.25, 3.5) node {\scriptsize $\rvdots$};
    \draw (3.5, 3.5) node [text=ForestGreen] {\scriptsize $\boldsymbol{\rvdots}$};
    \draw (4.75, 3.5) node {\scriptsize $\rvdots$};
    \draw (6, 3.5) node {\scriptsize $\rvdots$};
    % ---
    \draw (1, 2.5) node [text=DarkRed] {\tiny $\boldsymbol{F(\alpha_1, \alpha_i)}$};
    \draw (2.25, 2.5) node [text=DarkRed] {\scriptsize $\boldsymbol{\ldots}$};
    \draw (3.5, 2.5) node {\scriptsize $F(\alpha_i, \alpha_i)$};
    \draw (4.75, 2.5) node [text=DarkRed] {\scriptsize $\boldsymbol{\ldots}$};
    \draw (6, 2.5) node [text=DarkRed] {\tiny $\boldsymbol{F(\alpha_n, \alpha_i)}$};
    % ---
    \draw (1, 1.5) node {\scriptsize $\rvdots$};
    \draw (2.25, 1.5) node {\scriptsize $\rvdots$};
    \draw (3.5, 1.5) node [text=ForestGreen] {\scriptsize $\boldsymbol{\rvdots}$};
    \draw (4.75, 1.5) node {\scriptsize $\rvdots$};
    \draw (6, 1.5) node {\scriptsize $\rvdots$};
    % ---
    \draw (1, 0.5) node {\scriptsize $F(\alpha_1, \alpha_n)$};
    \draw (2.25, 0.5) node {\scriptsize $\ldots$};
    \draw (3.5, 0.5) node [text=ForestGreen] {\tiny $\boldsymbol{F(\alpha_i, \alpha_n)}$};
    \draw (4.75, 0.5) node {\scriptsize $\ldots$};
    \draw (6, 0.5) node {\scriptsize $F(\alpha_n, \alpha_n)$};
    % ---
    \draw (7.5, 4.5) node {\scriptsize $\boldsymbol{+}$};
    \draw (7.5, 3.5) node {\scriptsize $\rvdots$};
    \draw (7.5, 1.5) node {\scriptsize $\rvdots$};
    \draw (7.5, 0.5) node {\scriptsize $\boldsymbol{+}$};
    % ---
    \draw (8.5, 4.5) node {\scriptsize $r_{1i}$};
    \draw (8.5, 3.5) node {\scriptsize $\rvdots$};
    \draw (8.5, 1.5) node {\scriptsize $\rvdots$};
    \draw (8.5, 0.5) node {\scriptsize $r_{ni}$};
    % ---
    \draw (1, -0.5) node {\scriptsize $\boldsymbol{+}$};
    \draw (2.25, -0.5) node {\scriptsize $\ldots$};
    \draw (4.75, -0.5) node {\scriptsize $\ldots$};
    \draw (6, -0.5) node {\scriptsize $\boldsymbol{+}$};
    % ---
    \draw (1, -1.5) node {\scriptsize $r_{i1}$};
    \draw (2.25, -1.5) node {\scriptsize $\ldots$};
    \draw (4.75, -1.5) node {\scriptsize $\ldots$};
    \draw (6, -1.5) node {\scriptsize $r_{in}$};
    %% Polynomial (b)
    % Main rectangle
    \draw (11, 0) rectangle (18, 5);
    % Columns
    \draw (11, 2) -- (18, 2);
    \draw (11, 3) -- (18, 3);
    \draw (13.75, 0) -- (13.75, 5);
    \draw (15.25, 0) -- (15.25, 5);
    % Coloured Rectangles
    \draw [rounded corners, fill=ForestGreen!30] (19, 0) rectangle (21, 5);
    \draw [rounded corners, fill=DarkRed!30] (11, -2) rectangle (18, -1);
    % Annotations
    \draw (14.5, -4) node {\footnotesize (b)};
    \draw (14.5, -2.5) node [text=DarkRed] {\scriptsize $\WSS_i$};
    \draw (20, 5.5) node [text=ForestGreen] {\scriptsize $\WSS_j$};
    % ---
    \draw (10, 2.5) node {\footnotesize $f_i(x)$};
    \draw (10.7, 2.5) node {\footnotesize $\Rightarrow$};
    \draw (14.5, 6) node {\footnotesize $g_i(y)$};
    \draw (14.5, 5.5) node {\footnotesize $\Downarrow$};
    % ---
    \draw (12, 4.5) node {\scriptsize $F(\alpha_1, \alpha_1)$};
    \draw (13.25, 4.5) node {\scriptsize $\ldots$};
    \draw (14.5, 4.5) node [text=ForestGreen] {\tiny $\boldsymbol{F(\alpha_i, \alpha_1)}$};
    \draw (15.75, 4.5) node {\scriptsize $\ldots$};
    \draw (17, 4.5) node {\scriptsize $F(\alpha_n, \alpha_1)$};
    % ---
    \draw (12, 3.5) node {\scriptsize $\rvdots$};
    \draw (13.25, 3.5) node {\scriptsize $\rvdots$};
    \draw (14.5, 3.5) node [text=ForestGreen] {\scriptsize $\boldsymbol{\rvdots}$};
    \draw (15.75, 3.5) node {\scriptsize $\rvdots$};
    \draw (17, 3.5) node {\scriptsize $\rvdots$};
    % ---
    \draw (12, 2.5) node [text=DarkRed] {\tiny $\boldsymbol{F(\alpha_1, \alpha_i)}$};
    \draw (13.25, 2.5) node [text=DarkRed] {\scriptsize $\boldsymbol{\ldots}$};
    \draw (14.5, 2.5) node {\scriptsize $F(\alpha_i, \alpha_i)$};
    \draw (15.75, 2.5) node [text=DarkRed] {\scriptsize $\boldsymbol{\ldots}$};
    \draw (17, 2.5) node [text=DarkRed] {\tiny $\boldsymbol{F(\alpha_n, \alpha_i)}$};
    % ---
    \draw (12, 1.5) node {\scriptsize $\rvdots$};
    \draw (13.25, 1.5) node {\scriptsize $\rvdots$};
    \draw (14.5, 1.5) node [text=ForestGreen] {\scriptsize $\boldsymbol{\rvdots}$};
    \draw (15.75, 1.5) node {\scriptsize $\rvdots$};
    \draw (17, 1.5) node {\scriptsize $\rvdots$};
    % ---
    \draw (12, 0.5) node {\scriptsize $F(\alpha_1, \alpha_n)$};
    \draw (13.25, 0.5) node {\scriptsize $\ldots$};
    \draw (14.5, 0.5) node [text=ForestGreen] {\tiny $\boldsymbol{F(\alpha_i, \alpha_n)}$};
    \draw (15.75, 0.5) node {\scriptsize $\ldots$};
    \draw (17, 0.5) node {\scriptsize $F(\alpha_n, \alpha_n)$};
    % ---
    \draw (18.5, 4.5) node {\scriptsize $\boldsymbol{+}$};
    \draw (18.5, 3.5) node {\scriptsize $\rvdots$};
    \draw (18.5, 1.5) node {\scriptsize $\rvdots$};
    \draw (18.5, 0.5) node {\scriptsize $\boldsymbol{+}$};
    % ---
    \draw (12, -0.5) node {\scriptsize $\boldsymbol{+}$};
    \draw (13.25, -0.5) node {\scriptsize $\ldots$};
    \draw (15.75, -0.5) node {\scriptsize $\ldots$};
    \draw (17, -0.5) node {\scriptsize $\boldsymbol{+}$};
    % ---
    \draw (20, 4.5) node {\scriptsize $F_1^W(0, \alpha_1)$};
    \draw (20, 3.5) node {\scriptsize $\rvdots$};
    \draw (20, 1.5) node {\scriptsize $\rvdots$};
    \draw (20, 0.5) node {\scriptsize $F_n^W(0, \alpha_n)$};
    % ---
    \draw (12, -1.5) node {\scriptsize $F_i^W(0, \alpha_1)$};
    \draw (13.25, -1.5) node {\scriptsize $\ldots$};
    \draw (15.75, -1.5) node {\scriptsize $\ldots$};
    \draw (17, -1.5) node {\scriptsize $F_i^W(0, \alpha_n)$};
  \end{tikzpicture}
  \caption{Pictorial depiction of the construction of VSS from WSS. Part (a) depicts the masking of
    the common values to be broadcast by $P_i$ in Round II of the $\GIKR$-I scheme where random pads
    $r_{ij}$ (chosen by $P_i$) and $r_{ji}$ (received by $P_i$ from $P_j$) are used. In part (b) the
    construction of \cite{FGGRS06} is depicted where each party $P_i$ concurrently runs a WSS instance
    $\WSS_i$. $P_i$ masks values on its row polynomial (depicted in green) using points on
    $F_i^W(0, \alpha_j)$ where $P_j$ holds the row-polynomial $F_i^W(x, \alpha_j)$ of $P_i$'s blinding
    polynomial $h_i(x)$ shared using the instance $\WSS_i$. $P_i$ also masks values on its column
    polynomial (depicted in red) using points on the row-polynomial $F_j^W(\cdot, \alpha_i)$ of $P_j$'s
    instance $\WSS_j$ which is sharing $P_j$'s blinding polynomial $h_j(x)$ for $j \in \{1,\ldots,n\}$
    and $j \neq i$.}
\label{fig:WSSToVSS}
\end{figure}

==> SNThreshold.tex <==
\section{Preliminaries and Definitions}
\label{sec:SNThreshold}
%-----
The communication model considered in this part is the same as in part I, namely synchronous communication model where the parties are connected by pair-wise secure channels 
 and where the parties have access to a broadcast channel, with protocols operating as a sequence of rounds. However, 
 in the {\it non-threshold} model,  the corruption capability of $\Adv$ is specified by an adversary structure    $\AdvStructure = \{Z_1, \ldots, Z_q \} \subseteq
     2^{\Partyset}$, where   each $Z_m \subset \Partyset$ and where each $Z_m$ denotes a set of potentially corrupt nodes.
           The
   adversary $\Adv$ can corrupt a set of parties $Z^{\star} \subset \Partyset$   during
   the execution of a protocol, where $Z^{\star}$ is part of some set in the     adversary
structure (i.e., $Z^{\star} \subseteq Z_m$ for some $Z_m \in \AdvStructure$).  Note that the exact identity of the set
  $Z^{\star}$ will not be known to the honest parties at the beginning of the execution
   of any protocol, and need not be revealed even at the end of the protocol.
   The adversary structure $\AdvStructure$ is {\it monotone} in the sense that if $Z \in \AdvStructure$, then any $Z' \subseteq Z$ also belongs to 
   $\AdvStructure$. For convenience, we assume that $\AdvStructure$ consists of {\it maximal} subsets of parties, which can be potentially corrupted
   by $\Adv$ during the execution of a protocol.
    Following the terminology of \cite{HM00}, 
     we say that a set of parties $S \subseteq \Partyset$ satisfies the $\Q^{(k)}$ condition, if the union of any $k$ subsets from $\AdvStructure$ 
     {\it does not} cover the entire set $S$.
     That is, if $S \not \subseteq Z_1 \cup \ldots \cup Z_k$, for every
   $Z_1, \ldots, Z_k \in \AdvStructure$. Notice that if $S$ satisfies the $\Q^{(k)}$
   condition, then it also satisfies the $\Q^{(k')}$ condition for any $1 \leq k' < k$.
   It is easy to see that a threshold adversary is a special type of non-threshold adversary, where the corresponding adversary structure $\AdvStructure$
   consists of all possible $n \choose t $ subsets of $t$ parties among $\Partyset$. Consequently, in the non-threshold model 
   $\Partyset$ satisfies the $\Q^{(k)}$ condition, if and only if in the threshold model
    the condition $t < n/k$ holds.


==> symbols_env.tex <==
%--------------------------------------------------------------
%New Style boxes
%--------------------------------------------------------------



%----- Box Environment ---------------------------------------------------------
\RequirePackage{mdframed}

%Basic box structure with title box
\newenvironment{titlebox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.1\baselineskip,
		%skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		%skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=15pt}\setlist[enumerate]{leftmargin=15pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1.5em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

%title box style
\tikzstyle{normal} = [thick, fill=white, text=black, draw, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]
\tikzstyle{gray} = [thick, fill=gray!90, text=white, rounded corners, rectangle, minimum height=.7cm, inner sep=3pt]

%box style
\mdfdefinestyle{commonbox}{%
	%align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	%innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	%splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - 
	%innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
	%splittopskip=15pt,splitbottomskip=15pt
}


\mdfdefinestyle{roundbox}{style=commonbox,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{systembox}[3]
{\vspace{\baselineskip}\begin{titlebox}{Functionality \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{gsystembox}[3]
{\vspace{\baselineskip}\begin{titlebox}{Global Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}}
	
	

\newenvironment{protocolbox}[3]
{\begin{titlebox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}


\newenvironment{algobox}[3]
{\begin{titlebox}{Algorithm \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{reductionbox}[3]
{\begin{titlebox}{Reduction \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{gamebox}[3]
{\begin{titlebox}{Game \normalfont #1}{commonbox}{gray}{#2}{#3}}
	{\end{titlebox}}

\newenvironment{simulatorbox}[3]
{\begin{titlebox}{Simulator \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}}
%-------------------------------------------------------------------------------



%-------------------------------------------------------------------------------
%Split Box for IEETran Version
%-------------------------------------------------------------------------------
%Basic box structure with title box
\newenvironment{splittitlebox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.1\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

\mdfdefinestyle{commonsplitbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=5pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - 
	%innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
	%splittopskip=15pt,splitbottomskip=15pt
}

\newenvironment{protocolsplitbox}[3]
{\begin{splittitlebox}{Protocol \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}
	
\newenvironment{schemesplitbox}[3]
{\begin{splittitlebox}{Scheme \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}
	
	
\newenvironment{simulatorsplitbox}[3]
{\begin{splittitlebox}{Simulator \normalfont #1}{commonsplitbox}{normal}{#2}{#3}}
	{\end{splittitlebox}}	

%------------------------------------------------------------------------------
% Full Width Environments
%------------------------------------------------------------------------------

\newenvironment{systembox*}[3]
{\begin{strip}
\vspace{\baselineskip}\begin{titlebox}{Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{gsystembox*}[3]
{\begin{strip}
\vspace{\baselineskip}\begin{titlebox}{Global Functionality \normalfont #1}{roundbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{protocolbox*}[3]
{\begin{strip}
\begin{titlebox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{algobox*}[3]
{\begin{strip}
\begin{titlebox}{Algorithm \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{reductionbox*}[3]
{\begin{strip}
\begin{titlebox}{Reduction \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{gamebox*}[3]
{\begin{strip}
\begin{titlebox}{Game \normalfont #1}{commonbox}{gray}{#2}{#3}}
	{\end{titlebox}
\end{strip}}

\newenvironment{simulatorbox*}[3]
{\begin{strip}
\begin{titlebox}{Simulator \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{titlebox}
\end{strip}}




%------------------------------------------------------------------------------
%Basic box structure with mytitle box without embossed title
%------------------------------------------------------------------------------

%box style
\mdfdefinestyle{mycommonbox}{%
	align=center, middlelinewidth=1.1pt,userdefinedwidth=\linewidth
	innerrightmargin=0pt,innerleftmargin=2pt,innertopmargin=3pt,
	splittopskip=7pt,splitbottomskip=3pt
	%Actual Values - innerrightmargin=0pt,innerleftmargin=5pt,innertopmargin=5pt,
}
\mdfdefinestyle{myroundbox}{style=mycommonbox,roundcorner=5pt,userdefinedwidth=\linewidth}

\newenvironment{titlebox*}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=0.3\baselineskip,
		skipabove={0.4em},
		skipbelow={1em},needspace=3\baselineskip,
		frametitleaboveskip=5em,
		innerrightmargin=5pt
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1.5em}
	{\captionof{figure}{\normalfont \TitleCaption}\label{\TitleLabel}}
	\medskip
}

%------------------------------------------------------------------------------
% Box Environments without embossed title
%------------------------------------------------------------------------------

\newenvironment{mysystembox}[3]
{\begin{titlebox*}{Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mygsystembox}[3]
{\begin{titlebox*}{Global Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myprotocolbox}[3]
{\begin{titlebox*}{Protocol \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myalgobox}[3]
{\begin{titlebox*}{Algorithm \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{myreductionbox}[3]
{\begin{titlebox*}{Reduction \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mygamebox}[3]
{\begin{titlebox*}{Game \normalfont #1}{mycommonbox}{gray}{#2}{#3}}
	{\end{titlebox*}}

\newenvironment{mysimulatorbox}[3]
{\begin{titlebox*}{Simulator \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
	{\end{titlebox*}}
%-------------------------------------------------------------------------------


%------------------------------------------------------------------------------
% Full Width Environments without embossed title
%------------------------------------------------------------------------------

\newenvironment{mysystembox*}[3]
{\begin{strip}
		\vspace{\baselineskip}\begin{titlebox*}{Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mygsystembox*}[3]
{\begin{strip}
		\vspace{\baselineskip}\begin{titlebox*}{Global Functionality \normalfont #1}{myroundbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myprotocolbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Protocol \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myalgobox*}[3]
{\begin{strip}
		\begin{titlebox*}{Algorithm \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{myreductionbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Reduction \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mygamebox*}[3]
{\begin{strip}
		\begin{titlebox*}{Game \normalfont #1}{mycommonbox}{gray}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}

\newenvironment{mysimulatorbox*}[3]
{\begin{strip}
		\begin{titlebox*}{Simulator \normalfont #1}{mycommonbox}{normal}{#2}{#3}}
		{\end{titlebox*}
\end{strip}}






%-------------------------------------------------------------------------------
% Basic protocol box without Algohead NDSS
%-------------------------------------------------------------------------------
%Basic box structure with title box
\newenvironment{mytbox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.8\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-1.5em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

\newenvironment{mytsplitbox}[5]
{\mdfsetup{
		style=#2,
		innertopmargin=1.8\baselineskip,
		skipabove={\dimexpr0.2\baselineskip+\topskip\relax},
		skipbelow={1em},needspace=3\baselineskip,
		singleextra={\node[#3,right=10pt,overlay] at (P-|O){~{\sffamily\bfseries #1 }};},%
		firstextra={\node[#3,right=10pt,overlay] at (P-|O) {~{\sffamily\bfseries #1 }};},
		frametitleaboveskip=9em,
		innerrightmargin=5pt
		%skipabove={\dimexpr0.7\baselineskip+\topskip\relax},
	}
	\newcommand{\TitleCaption}{#4}
	\newcommand{\TitleLabel}{#5}
	\begin{mdframed}[font=\small]
		\setlist[itemize]{leftmargin=13pt}\setlist[enumerate]{leftmargin=13pt}\raggedright% 
	}
	{\end{mdframed}
	\vspace{-0.8em}
	{\captionof{figure}{\small \TitleCaption}\label{\TitleLabel}}
	\medskip
}

\newenvironment{mypbox}[3]
{\begin{mytbox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{mytbox}}

\newenvironment{mypsplitbox}[3]
{\begin{mytsplitbox}{Protocol \normalfont #1}{commonbox}{normal}{#2}{#3}}
	{\end{mytsplitbox}}











%-------------------------------------------------------------------------------
% Macros used for the examples
%-------------------------------------------------------------------------------

%----- Algorithm Environment ---------------------------------------------------
%Header for Algorithms/Functionalities
\newcommand{\algoHead}[1]{\vspace{0.2em} \underline{\textbf{#1}} \vspace{0.3em}}
\newcommand{\algoHeadN}[1]{\vspace{0.2em} \textbf{#1} \vspace{0.3em}}
\newcommand{\algoHeadExt}[2]{\vspace{0.2em} \underline{\textbf{#1} #2} \vspace{0.3em}}

%Multiline Algo-States
\makeatletter
\algnewcommand{\ExtendedState}[1]{\State
	\parbox[t]{\dimexpr\linewidth-\ALG@thistlm}{\hangindent=\algorithmicindent\strut\hangafter=3#1\strut}}
\makeatother

%Algorithms States
\algnewcommand\algorithmicinput{\textbf{Input:}}
\algnewcommand\Input{\item[\algorithmicinput]}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

%Algo Comments
\algrenewcommand{\algorithmiccomment}[1]{{\color{gray}// #1}}
